Pixtral 12B

We introduce Pixtral-12B, a 12--billion-parameter multimodal language model. Pixtral-12B is trained to understand both natural images and documents, achieving leading performance on various multimodal benchmarks, surpassing a number of larger models. Unlike many open-source models, Pixtral is also a cutting-edge text model for its size, and does not compromise on natural language performance to excel in multimodal tasks. Pixtral uses a new vision encoder trained from scratch, which allows it to ingest images at their natural resolution and aspect ratio. This gives users flexibility on the number of tokens used to process an image. Pixtral is also able to process any number of images in its long context window of 128K tokens. Pixtral 12B substanially outperforms other open models of similar sizes (Llama-3.2 11B \& Qwen-2-VL 7B). It also outperforms much larger open models like Llama-3.2 90B while being 7x smaller. We further contribute an open-source benchmark, MM-MT-Bench, for evaluating vision-language models in practical scenarios, and provide detailed analysis and code for standardized evaluation protocols for multimodal LLMs. Pixtral-12B is released under Apache 2.0 license.

==> tables/standard_devs.tex <==
% Define colors (if not already defined)
\definecolor{flexOne}{RGB}{199,232,229}   % Lighter Teal for Mathvista
\definecolor{flexTwo}{RGB}{239,245,214}   % Lighter Light green for MMMU
\definecolor{flexThree}{RGB}{253,224,175} % Lighter Orange for ChartQA
\begin{table}[htbp]
\centering
\small
\begin{tabular}{@{}lccc@{}}
\toprule
& \multicolumn{1}{c}{\cellcolor{flexOne}\textbf{Mathvista}} & \multicolumn{1}{c}{\cellcolor{flexTwo}\textbf{MMMU}} & \multicolumn{1}{c}{\cellcolor{flexThree}\textbf{ChartQA COT}} \\
\cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4}
Model $\longrightarrow$ & Flexible Level 3 & Flexible Level 3 & Flexible Level 3 \\
\midrule
Llama-3.2 11B~\cite{touvron2023llama} & 42.1 {\scriptsize\textcolor{gray}{($\pm$1.9)}} & 45.3 {\scriptsize\textcolor{gray}{($\pm$1.0)}} & 77.2 {\scriptsize\textcolor{gray}{($\pm$0.8)}} \\
Llama-3.2 90B~\cite{touvron2023llama} & 55.6 {\scriptsize\textcolor{gray}{($\pm$1.5)}} & 55.9 {\scriptsize\textcolor{gray}{($\pm$0.5)}} & 80.1 {\scriptsize\textcolor{gray}{($\pm$0.5)}} \\
Qwen2-VL 7B~\cite{wang2024qwen2vlenhancingvisionlanguagemodels} & 53.7 {\scriptsize\textcolor{gray}{($\pm$2.1)}} & 46.9 {\scriptsize\textcolor{gray}{($\pm$1.9)}} & 77.0 {\scriptsize\textcolor{gray}{($\pm$0.8)}} \\
Pixtral 12B & \textbf{56.4} {\scriptsize\textcolor{gray}{($\pm$1.0)}} & \textbf{49.5} {\scriptsize\textcolor{gray}{($\pm$1.5)}} & \textbf{84.0} {\scriptsize\textcolor{gray}{($\pm$0.4)}} \\
\bottomrule
\end{tabular}
\vspace{1mm}
\caption{\textbf{Flexible Level 3 performance across datasets.} 
All values are multiplied by 100 and rounded to one decimal place. 
The highest score for each dataset is in bold.
Flexible Level 3 is included for illustration only, as it allows some incorrect answers to be marked as correct.
}
\label{tab:flexible_level_3}
\end{table}
